Cross-lingual Intermediate Fine-tuning improves Dialogue State Tracking

Recent progress in task-oriented neural dialogue systems is largely focused on a handful of languages, as annotation of training data is tedious and expensive. Machine translation has been used to make systems multilingual, but this can introduce a pipeline of errors. Another promising solution is using cross-lingual transfer learning through pretrained multilingual models. Existing methods train multilingual models with additional code-mixed task data or refine the cross-lingual representations through parallel ontologies. In this work, we enhance the transfer learning process by intermediate fine-tuning of pretrained multilingual models, where the multilingual models are fine-tuned with different but related data and/or tasks. Specifically, we use parallel and conversational movie subtitles datasets to design cross-lingual intermediate tasks suitable for downstream dialogue tasks. We use only 200K lines of parallel data for intermediate fine-tuning which is already available for 1782 language pairs. We test our approach on the cross-lingual dialogue state tracking task for the parallel MultiWoZ (English -> Chinese, Chinese -> English) and Multilingual WoZ (English -> German, English -> Italian) datasets. We achieve impressive improvements (> 20% on joint goal accuracy) on the parallel MultiWoZ dataset and the Multilingual WoZ dataset over the vanilla baseline with only 10% of the target language task data and zero-shot setup respectively.

==> multiwoz_example.tex <==
\begin{table*}[]
\small
\centering
\begin{tabular}{|l|l|}
\hline
Interaction                                                                                                                                                      & Dialogue State                                                                                                                \\ \hline
User:  I need to book a hotel in the east that has 4 stars.                                                                                                         & \{hotel-inform-area: east, hotel-inform-stars: 4\}                                                                            \\ \hline
\begin{tabular}[c]{@{}l@{}}System: I can help you with that. What is your price range?\\ User: That doesn't matter as long as it has free wifi and parking.\end{tabular} & \begin{tabular}[c]{@{}l@{}}\{hotel-inform-area: east, hotel-inform-stars: 4,\\hotel-inform-parking: yes, hotel-inform-wifi: yes,\\ hotel-inform-price: dontcare\}\end{tabular} \\ \hline
\end{tabular}
\caption{An example of interaction and the corresponding user dialogue state in MultiWoZ 2.1. The dialogue state consists of slot-types and slot-values. Note that the slot type follows \{domain\}-\{user\_intent\}-\{slot\_name\} format. }
\label{tab:multiwoz_example}
\end{table*}
